Electricity Load and Peak Forecasting: Feature Engineering, Probabilistic LightGBM and Temporal Hierarchies

We describe our experience in developing a predictive model that placed high position in the BigDeal Challenge 2022, an energy competition of load and peak forecasting. We present a novel procedure for feature engineering and feature selection, based on cluster permutation of temperatures and calendar variables. We adopted gradient boosting of trees and we enhance its capabilities with trend modelling and distributional forecasts. We also include an approach to forecast combination known as temporal hierarchies, which further improves the accuracy.

==> DistributionalForecastswithLightGBM.tex <==
% LightGBM  returns only a point forecasts, i.e. it returns the  conditional mean $\mathbb{E}(Y\,|\,\mathbf{X}=\mathbf{x})$. 
% However, any decision making requires the whole conditional distributions $F_Y(y\,|\,\mathbf{x})$.
% März et al. \cite{Marz2022} propose a  probabilistic extension of  XGBoost, which predicts the moments of  conditional distribution $F_Y(y\,|\,\mathbf{x})$, thus solving the problem of quantile crossing.

% In \cite[Sec. II,A]{Marz2022}, distributional modelling is formulated as follows:
% \begin{equation}
%     y_i \stackrel{ind}{\sim} \mathcal{D}
%     \left(
%     \begin{aligned}
%          & h_1(\theta_{i1} = \eta_{i1} \\
%          & h_2(\theta_{i2} = \eta_{i2} \\
%          & \quad \quad \quad \vdots \\
%          & h_K(\theta_{iK} = \eta_{iK}
%     \end{aligned}
%     \right)
%     \label{eq:distrlearning}
% \end{equation}
% for $i = 1,\ldots,n$, where $\mathcal{D}$ denotes a parametric distribution for the response $\mathbf{y}$ that depends on $K$ distributional parameters $\theta_k$, $k=1,\ldots, K$, and with $h_k(\cdot)$ denoting a known function relating distributional parameters to predictors $\eta_k$. In its most generic form, the predictors $\eta_k$ are given by
% \begin{equation}
%     \eta_k = f_k(x), \quad \quad k=1,\ldots,K
%     \label{eq:distrlearning_predictors}
% \end{equation}

% Predictors in \eqref{eq:distrlearning_predictors} can by learned from tree-based models which relies on the availability of first and second-order derivatives of the log-likelihood (e.g. LighGBM implements the second-order Taylor expansion). Hence, the distributional parameters $\theta_k$ are estimated via maximum likelihood estimation (MLE) where a separate tree is grown for each $\theta_k$.

==> GradientBoostingandLightGBMmodel.tex <==
% \paragraph{Gradient Boosting}Gradient Boosting (GB) \cite{friedman2001greedy} is a machine learning algorithm that uses an ensemble of weak learners; in the following we show  the  formulation with decision-trees. Given a dataset $\mathcal{D}=\{(x_i,y_i)\}_{i=1}^{n}$ and a differentiable loss function $L(y_i,F(x))$, the model is initialized with a constant value:
% \begin{equation}
%     F_0(x) = \arg \min_{\gamma} \sum_{i=1}^{n}{L(y_i,\gamma})
%     \label{eq:gb_1}
% \end{equation}
% Let $M$ be the number of weak learners. At each step $m$: \\(a) pseudo-residuals $r_{i,m}$ are computed, for $i=1,\ldots,n$:
% \begin{equation}
%     r_{i,m} = - \bigg [\frac{\partial L(y_i, F_{m-1}(x_i))}{\partial F_{m-1}(x_i)} \bigg]
%     \label{eq:gb_2}
% \end{equation}
% (b) a weak learner is fitted to predict $r_m$ and create terminal regions $R_{j,m}$ (i.e. the leaves). \\(c) for $j=1,\ldots,J_m$ the \textit{output value} is computed for each region, as in \eqref{eq:gb_1} but also considering previous prediction:
% \begin{equation}
%     F_{j,m}(x) = \arg \min_{\gamma} \sum_{x_i \in R_{i,j}}{L(y_i,F_{m-1}(x_i)+\gamma})
%     \label{eq:gb_3}
% \end{equation}
% (d) $\eta \in [0,1]$ is the learning rate, new predictions are computed by:
% \begin{equation}
%     F_{m}(x) = F_{m-1}(x) + \eta F_m(x)
%     \label{eq:gb_4}
% \end{equation}

%  \paragraph{GB Frameworks} XGBoost (eXtreme Gradient Boosting) \cite{chen2016xgboost}
%  is a popular implementation of GB with decision-trees 
%  which uses a second-order Taylor expansion \eqref{eq:xgboost_2} to solve the optimal \textit{output value} equation, defined  as the sum of the loss functions and the regularization terms: 
% \begin{equation}
%     \textbf{Obj}:\,\, \arg \min_{\gamma} \bigg[\sum_{i \in I_j}L(y_i,F_{m-1}(x_i)+\gamma)  \bigg] + \rho T_{m} + \frac{1}{2}\lambda\gamma
%     \label{eq:xgboost_1}
% \end{equation}
% \begin{equation}
%     L(y_i, z_i+\gamma) \approx L(y_i,z_i) + \underbrace{\frac{\partial L(y_i,z_i)}{\partial z_i}}_{\text{Gradient}\,\,g_i}\gamma + \frac{1}{2}\underbrace{\frac{\partial^2 L(y_i,z_i)}{\partial z_i^2}}_{\text{Hessian}\,\,h_i}\gamma^2
%     \label{eq:xgboost_2}
% \end{equation}
% where $I_j$ is the set of all samples in leaf $j$, $F_{m-1}(x_i) = z_i$, $T$ is the number of leaves in a tree, $\rho$ is a penalty factor meant for pruning, and $\lambda > 0$ shrinks the optimal output value to 0. Equation \eqref{eq:xgboost_1} and the similarity score used to grow the tree are closed-form functions of gradients and hessians. 

% XGBoost has become a de-facto machine learning model for winning competitions. However, it has heavy computational requirements. LightGBM \cite{ke2017lightgbm} is a more recent algorithm implementation which provides comparable accuracy, but with faster training, low memory usage and scalability with large datasets. By design XGBoost grows deep-wise trees, while LightGBM grows leaf-wise trees. 

% \paragraph{DART}
% Gradient boosting is subject to overfitting, since the last estimators focus only on a small subset of the training data.
% The DART algorithm
% (Dropouts meet Multiple Additive Regression Trees) \cite{Korlakai2015} solves the problem.
% When computing the gradients, DART selects a random subset of $k$ previous estimators. 
% DART boosting engine is implemented within the LightGBM framework.

==> Performancemeasures.tex <==
% \hl{da portare nella parte di esperimenti. }
% We evaluate the forecasting performance  of both point forecasts and prediction intervals. 

% We score the point forecasts using
% the \textit{Mean Absolute Percentage Error} (MAPE):
%  %is defined as:%(MAPE) computes the percentage deviations between forecasted loads and actual loads, with respect to actual loads. Since it is a scale independent metric, i.e. it scales the quantities in percentage units, it allows for comparison between time series with different loads (where the quantities are in MW/h). 
% \begin{equation}
%     \text{MAPE} = \frac{1}{h}\sum_{t=T+1}^{T+H}{\frac{|y_t - \hat{y}_t|}{|y_t|} \times 100 },
%     \label{eq:mape}
% \end{equation}
% where $T$ denotes the time of the last observation, $y_t$ and $\hat{y}_t$ denote the actual value and the point forecast for time $t$.

% MAPE has been used by the BigDeal competition to score the point forecasts. However,  it has some important  drawbacks: it is numerically unstable if $y_t$ is close to 0, and it  is biased since it penalizes more over-estimation than under-estimation error \cite{Armstrong1992}.
% Furthermore, it is bounded to $100\%$ for under-estimated forecasts but it is unbounded for over-estimated forecasts. To be more robust on these issues the literature \cite{Chen2004, hyndMAPE} propose the \textit{Symmetric Mean Absolute Percentage Error} (sMAPE).
% % , as described in \eqref{eq:smape}, also used in this work.
% % \begin{equation}
% %     \text{sMAPE} = \frac{1}{h}\sum_{t=T}^{h}{\frac{2|y_t - \hat{y}_t|}{|y_t|+|\hat{y}_t|}}
% %     \label{eq:smape}
% % \end{equation}
% %
% % As a third metric for point forecast we used the \textit{Root mean squared error} (RMSE), as described in \eqref{eq:rmse}.
% % \begin{equation}
% %     \text{RMSE} = \sqrt{\frac{1}{h}\sum_{t=T}^{h}{(y_t - \hat{y}_t)^2}}
% %     \label{eq:rmse}
% % \end{equation}

% \paragraph{Predictive distribution}
% To evaluate the predictive distribution we use the  \textit{Energy Score} (ES) \cite{Gneiting2007}, a multivariate generalization of the Continuous Ranked Probability Score (CRPS). Let $\mathbf{y}$ be the actual multivariate observation, and given $k$ samples $\mathbf{x}_1, \mathbf{x}_2,\ldots,\mathbf{x}_k$ from the multivariate predictive distribution $\mathbf{F}$. The Energy Score is defined as:
% \begin{equation}
%     \text{ES}(\mathbf{F},\mathbf{y}) = \frac{1}{k}\sum_{i=1}^{k}\norm{\mathbf{y}-\mathbf{x}_i}^{\alpha} - \frac{1}{2k^2}\sum_{i=1}^{k}\sum_{j=1}^{k}\norm{\mathbf{x}_i-\mathbf{x}_j}^{\alpha}\,.
%     \label{eq:es}
% \end{equation}
% We compute energy score using the \texttt{scoringRules} R package \cite{scoringRules}, with $\alpha=2$.

%  \textit{Interval Score} (IS) \cite{gneiting2011quantiles}. Given a forecast distribution, we denote by $1-\alpha$ the desired coverage of the interval, by $\mathbf{l}$ and $\mathbf{u}$ the lower and upper bounds of the interval. The score penalizes large intervals and intervals which do not contain the actual value. We consider a $90\%$ of coverage, with $\alpha=0.1$. We have:
% \begin{equation}
%     \text{IS}(\mathbf{l},\mathbf{u},\mathbf{y})= (\mathbf{u}-\mathbf{l}) + \frac{2}{\alpha}(\mathbf{l}-\mathbf{y})\mathbbm{1}(\mathbf{y} < \mathbf{l}) + \frac{2}{\alpha} (\mathbf{y}-\mathbf{u}) \mathbbm{1}(\mathbf{y} > \mathbf{u})\,.
% \end{equation}

% With a $90\%$ coverage we also report the mean interval width (IW) and the percentage of times the actual value is contained (IC). 


% We calculated previous metrics over the whole $h$, hence evaluating the forecasted loads at each hourly time-step. Daily peaks forecasts are evaluated with Magnitude, Timing and Shape measures described in Sec. \nameref{sec:bigdeal_challenge}, plus ES for the uncertainties.

% \paragraph{\textit{Skill score}}Let $m_{origin}$ and $m_{new}$ two comparable metrics. We denote the positive or negative percentage improvement by the Skill score defined as:
% \begin{equation}
%     \textbf{Skill}_{\%}(m_{origin},m_{new}) = \frac{m_{origin} - m_{new}}{(m_{origin} + m_{new})/2} \times 100
%     \label{eq:improvement}
% \end{equation}
